Tempo Adaptation in Non-stationary Reinforcement Learning

We first raise and tackle a ``time synchronization'' issue between the agent and the environment in non-stationary reinforcement learning (RL), a crucial factor hindering its real-world applications. In reality, environmental changes occur over wall-clock time ($t$) rather than episode progress ($k$), where wall-clock time signifies the actual elapsed time within the fixed duration $t \in [0, T]$. In existing works, at episode $k$, the agent rolls a trajectory and trains a policy before transitioning to episode $k+1$. In the context of the time-desynchronized environment, however, the agent at time $t_{k}$ allocates $\Delta t$ for trajectory generation and training, subsequently moves to the next episode at $t_{k+1}=t_{k}+\Delta t$. Despite a fixed total number of episodes ($K$), the agent accumulates different trajectories influenced by the choice of interaction times ($t_1,t_2,...,t_K$), significantly impacting the suboptimality gap of the policy. We propose a Proactively Synchronizing Tempo ($\texttt{ProST}$) framework that computes a suboptimal sequence {$t_1,t_2,...,t_K$} (= { $t_{1:K}$}) by minimizing an upper bound on its performance measure, i.e., the dynamic regret. Our main contribution is that we show that a suboptimal {$t_{1:K}$} trades-off between the policy training time (agent tempo) and how fast the environment changes (environment tempo). Theoretically, this work develops a suboptimal {$t_{1:K}$} as a function of the degree of the environment's non-stationarity while also achieving a sublinear dynamic regret. Our experimental evaluation on various high-dimensional non-stationary environments shows that the $\texttt{ProST}$ framework achieves a higher online return at suboptimal {$t_{1:K}$} than the existing methods.

==> files/1_intro_old.tex <==
\section{Introduction}

%% ========== old files ===========
\begin{comment} 
Over the last decades, reinforcement leaning (RL)  \citep{sutton1998rli} has been successful \cite{mnih2013playing,Silver2016MasteringTG}. Most of these works assume that the agent learns an optimal policy that maximizes the expected return for a given \textit{stationary} Markov decision process (MDP) with unknown reward and transition function. However, in the real world, that assumption is no longer valid \cite{zhu2020transfer}, and existing works face a restriction on extending their work  to solve practical problems of interest where environments are \textit{non-stationary} \cite{dulac2019challenges,padakandla2021survey}. One of the critical challenges that prevents classical RL algorithms from being generalized to non-stationary MDPs is their inability to quickly adapt to changing environments \cite{chen2022adaptive,huang2021adarl,feng2022factored,zintgraf2019varibad}. Adapting to environmental changes is a significant requirement for many real-world applications, but current state-of-the-art RL methods still struggle with this task.
\yuhao{Why exploitation \& exploration is not enough for non-stationary RL? Then we introduce what is tempo and why it is important.}
In non-stationary RL, agents must find a good strategy that balances the triad among exploitation, exploration, and \textbf{adaptation}, which adds an additional perspective to the classical RL problem of exploration-exploitation trade-offs.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/motivation_2dreacher.png}
    \caption{(a) 2D goal reacher in time-varying environment (b) forecasted model-based synthetic trajectories (c) Rewards per episode in 2D goal reacher with four model-free baselines. F-MBPO$^{*}$ is our proposed method }
    \label{fig:fig1}
\end{figure}

\yuhao{Limitations of existing work: Although the importance and ubiquity of non-stationary RL, the existing works have drawbacks.
(1) The first limitation is the passive estimation of the non-stationary environments. Most theoretical work [abcd] only focuses on the sliding window based estimator and neglects the forecastability of the underlying system. (2) The second issue is how to model the non-stationarity. [abcd] focus on directly forecasting the non-stationary policy gradient to adapt the time-varying optimal policies, which have problems of unstable learning, and uncertainty of performance. (3) Furthermore, since the agent can only execute a policy in a fixed environment once due to the non-stationary of the environments,  most existing work only updates the policy once for each environment which prevents the tracking of the time-varying optimal policies.}

% Most model-free adaptation strategies focus on how to provide a good gradient direction to obtain the time-varying optimal policy. However, optimizing a non-stationary empirical loss comes from time-varying data distribution have problems of unstable learning, uncertainty of performance [abcd].

To illustrate the limitations of the existing methods, let's take a toy example that a robot stated at the origin $O$ is given a task to reach inside a gray-shaded target box where its position is changing as time goes by (Figure \ref{fig:fig1}-(a)). 

\yuhao{The toy example results should support the limitations we mentioned for the existing works. Briefly discuss the bad empirical performance of existing methods}


\yuhao{However, } after the robot finishes execution at episode 10, if the robot can $observe$ how the box changes at episode 7 to 10, then predicts its position of next episode, then the robot can obtain good $\pi_{11}$ \textit{in advance} at current episode 10. That is, the robot's strategy is that rather than directly solves the non-stationary optimization problem, it proactively foresees where the next episode's target box will be located and solves the  stationary optimization in that created forecasted environment.
\yuhao{Also mention that: if we can generate synthetic trajectories from the forecasted models to optimize policy}

\yuhao{As motivated by this example, we aim to develop a systematic approach to fully leverage the proactive model forecaster and the synthetic samples from the forecasted envirments to get the optimal future policy in advance at current episode}

% \yuhao{ (research question) In this paperwe are interested in answering the following question: can model-based model-free framework with the proactive forecaster improve the existing work }

% This strategy well demonstrates our idea : \textit{Predicts future reward, transition probability of next episode and get optimal future policy in advance at current episode}.

Our idea, utilizing the forecasted environments to generate synthetic samples for policy optimization, is \hyunin{more prestigious }than the existing works \cite{chandak2020optimizing,al2017continuous,finn2019online} (figure \ref{fig:fig1}-(b)), which is well-supported by simulation results of 2D goal reacher in figure \ref{fig:fig1}-(c) . In the non-stationary environment, the agent usually obtain a trajectory from the current environment since the environment is keeping changing, which is challenging to optimize the policy using only a single trajectory. To solve this issue, if the agent updates its policy based on historical trajectories in a non-stationary environment, a lag between the environment that the agent have interacted with and the environment that the agent have to optimized in leads to inaccurate estimation of loss function and yields undesired policy. 
However, if the agent is able to maintain an accurate foresight of the future environment and utilize the forecasted environment to generate the multiple synthetic trajectories, then the foresight of the environment and unlimited number of synthetic trajectories will empower the agent to adapt its policy quickly for every future environment. Namely, a more accurate forecasting the future environment, much lower the model prediction error between forecasted environment and true future environment, then multiple samples from forecasted environment  enables the agent to optimize policy multiple iterations for each certain environment, which reduces the optimallity gap compared with the one-step policy optimization method. Those two in combination can provide a tighter dynamic regret. We elaborate specific details in Appendix \ref{appendix: 2D reacher environment setting}, \ref{appendix : Theoretical_Motivation}.  \yuhao{after introducing tempo, you may also need to mention tempo in this paragraph.}


% In online decision making, the agent should maintain good sample-efficiency that guarantees sub-optimal policy \cite{Foster2021TheSC}. 

% To motivate why forecasting the environment is more prestigious than directly model-free method, we give an example with one-link robot. We simplify the figure 1 setting to one link robot arm that only executes 1 step to reach the shaded area. We denote $s$ as the rotation angle of the link, and $a$ as a torque value of the origin joint. Discrete into tabular setting, $\mathcal{S} = \{1^{\circ},2^{\circ},..,90^{\circ} \}$ as an possible angle, and $\mathcal{A} = \{a_{1^{\circ}},a_{1^{\circ}},..,a_{90^{\circ}}\}$ where $a_{s}$ denotes the torque action that rotates $s$ degree, namely $s_{1} = s_{0} + s $ when executing $a_s$, and time varying $\mathcal{R}^k = \{+1 \text{ if } s_1 =k \text{ o.w. }0\}$ where represents that the shaded area is defined as $s=k$ where $k$ is episode. The robot always starts $s_0 =0^{\circ}$. In this setting, the episode changes from $1,2,..,90$, and the agent always get an $+1$ reward if agent can choose the action $a_{k}$ at episode $k$.Namely, the optimal action at episode $k$ is $a_{k^\circ}$.

% Now, let the value function $V(\pi^k) = \sum_{a\in\mathcal{A}}(r^k(s_0,a)\pi^k(a|s_0))$. Now let's assume at episode $k$, the agent learned the optimal policy $\pi^{*,k}(a|s_0) = \mathbbm{1}(a = a_{k^\circ})$. Now it plans to use it as next episode's policy $\pi^{k+1}$, then the agent moves to next episode $k+1$. The agent estimates the value function $V(\pi^{k+1})$ to get the optimal policy , but $V(\pi^{k+1}) =0$ since now $r^{k+1}(s_0,a_{k^{\circ}}) =0 $ and  $r^{k+1}(s_0,a_{{k+1}^{\circ}}) =+1$. So the agent's policy get zero gradient and maintain same policy with $\pi^{*,k}$ for all episodes after episode $k$. 

% However, now let us assume situation that the agent now forecasts the future reward function. Also assume the agent learned the optimal policy $\pi^{*,k}$. At the end of episode $k$, if the agent accurately predicts next episode $\hat{r}^{k+1}(s_0,a) = \mathbbm{1}(a = a_{k+1^{\circ}})$ and do several gradient descent steps of $\partial V(\pi^k) / \partial \theta$ to get $\pi^{k+1}$, the agent always gets positive gradient signal on $a=a_{k+1}$. So good prediction of future reward provides a good signal to induce the policy to execute $a=a_{k+1}$ at next episode.  


% Our research question driving this study is based on the following problem: previously proposed algorithms, which combine model-based and model-free methods \cite{janner2019trust}, should be re-examined in non-stationary environments. The advantage of the model-free method is its computational efficiency, allowing for direct learning of complex policies from raw data \cite{Mnih2015HumanlevelCT,lillicrap2015continuous}, while the advantage of the model-based method is its data efficiency, allowing one to learn fast by learning how the environment works \cite{sun2018dual,luo2018algorithmic}. However, both advantages are weakened in non-stationary environments since the time-varying trajectory distribution makes the model-free method challenging to obtain the optimal policy \cite{fei2020dynamic,chandak2020towards} and the model-based method challenging to minimize an additional model error term \cite{ding2022non,cheung2020reinforcement}. This problem leads us to the research question,
% \begin{center}
%     \textit{
%     How to flexibly combine the model-free and model-based method that achieves good balance among exploitation, exploration, and adaption?
%     }
% \end{center}

% Our idea to address this question starts from reexamining the fundamental reason why adaption should be fast. The term ``adaption'' implies the need to reduce the gap between the current environment, where the agent is optimizing its policy, and the future environment, where it will execute the optimized policy. The "fast adaptation" is necessary because its gap is unfathomable. This inspection provides a key idea to our research question, adopting a hybrid approach that incorporates model-based proactive model to forecast what the future environment will look like while using model-free methods to update the policy.

In this paper, we propose a fast adaptation strategy, \textbf{proactive model-based model-free} meta framework, that can be applied with any classical RL algorithm. The proposed meta framework is characterized by three key features: 1) it is \textit{proactive} in nature as it forecasts the future MDP; 2) it is \textit{model-based} by creating a synthetic future MDP; then 3) it is \textit{model-free} by directly optimizing the policy in the synthetic environment and using it in the subsequent future episode. To deeply understand and characterize our meta framework, we further propose two specific instances of our proposed meta framework : \textbf{FT-MBPO}, a theoretical instance for tabular environments, and \textbf{F-MBPO}, the practical instance for complex environments. 

The contribution of our work is listed below.
\begin{enumerate}
    \item \textbf{Generality : } our meta framework to cope with non-statinoary environments that could be equipped with RL algorithms. This is supported by Theorem \ref{thm:2}, Remark \ref{rmk:W-LSE_modelerror}.
    \item \textbf{Theoretical analysis (Section \ref{From_FT-MBPO_to_F-MBPO}): }
    \begin{itemize}
        \item we provide the dynamic regret of FT-MBPO in Theorem \ref{thm:forecasteddynamicregret}.
        \item we show that a good baseline RL algorithm is not enough to obtain sublinear dynamic regret in Proposition \ref{proposition:1} by pointing out that dynamic regret depends on our meta framework in Remark $\ref{remark:1}$.
        \item we show the dynamic regret achieves sublinearity when using the well-known non-stationary estimator in Theorem \ref{thm:2}, and can be more improved by a more general non-stationary estimator that includes a joint-optimization problem in Remark \ref{rmk:W-LSE_modelerror}.
    \end{itemize}
    \item \textbf{Practical implementation (Section \ref{experiments}): }
   
    \begin{itemize}
        \item  we conduct experiments of F-MBPO on three different Mujoco tasks and verify that our meta framework can quickly adapt and outform than the $\{\text{proactive, reactive}\}$-model-free methods proposed to solve the non-stationary MDPs and the typical model-based model-free method proposed to solve the statinoary MDPs.
    \end{itemize}
\end{enumerate}

This paper is organized as follows. Section \ref{problem_statement_and_background} provides the necessary background on non-stationary MDPs. In section \ref{method}, we introduce our main contribution, the meta framework that forecasts future MDPs. In section \ref{From_FT-MBPO_to_F-MBPO}, we then present two specific algorithms, FT-MBPO and F-MBPO, and provide theoretical analysis that leads to practical insights for algorithm design. Finally, we present our experimental results in section \ref{experiments}.
\end{comment}
%% ================================

Over the last decades, reinforcement leaning (RL)  \citep{sutton1998rli} has been successful \cite{mnih2013playing,Silver2016MasteringTG}. Most of these works assume that the agent learns an optimal policy that maximizes the expected return for a given \textit{stationary} Markov decision process (MDP) with unknown reward and transition function. However, in the real world, that assumption is no longer valid \cite{zhu2020transfer}, and existing works face a restriction on extending their work to solve practical problems of interest where environments are \textit{non-stationary} \cite{dulac2019challenges,padakandla2021survey}. One of the critical challenges that prevents classical RL algorithms from being generalized to non-stationary MDPs is their inability to quickly adapt to changing environments \cite{chen2022adaptive,huang2021adarl,feng2022factored,zintgraf2019varibad}. Adapting to environmental changes is a significant requirement for many real-world applications, but current state-of-the-art RL methods still struggle with this task. 

However, \hyunin{none of the research} have theoretically and practically investigated how to control \textbf{adapt to adapt}, that is the \textbf{tempo} of the adaption. We define tempo as the pace of all the processes that happen in a non-stationary environment. For example, a tempo of the environment means how fast the environment changes as time goes by, a tempo of the policy update means how many times you update the policy to behave well in the current environment, and a tempo of the model update means how many times you update the model to fit the current environment.

Why considering the tempo of adaptation in a non-stationary environment is important? In this paper, we raise the problem that \textit{non-stationary RL involves a hidden trade-off problem between the tempo of an algorithm and the tempo of the environment } and claim that \textbf{finding a good tempo trade-off between algorithm and time-varying environment is significant for adaptation}. For example, in the model-free method in non-stationary RL, a trade-off between the tempo of policy optimization and the tempo of environment exists. If the environment changes slowly, then a large number of iterations of policy optimization helps the agent keep track of time-varying optimal policies, but if the environment changes fast, then large optimization iterations can make the agent stuck in the one of past optimal policies and hard to adapt to new policy as episode goes by. Furthermore, in model-based model-free method in non-stationary RL, the triad among the tempo of policy optimization, the model optimization, and the tempo of environment exists. If the environment changes slowly, then the agent can both increase iteration of policy optimization and that of model optimization to fast adapt the optimal policy, but still a trade-off between policy optimization tempo and model optimization tempo exists. If the environment changes fast, then the agent should decrease the policy update pace and the model update pace, but the trade-off between the two still exists. Namely, the environment tempo affects the baseline tempo trade-off between policy optimization and model optimization to stay in high or low tempo. 

Although there are some existing works that achieve fast adaptability in non-stationary RL, those still have drawbacks that should be addressed regarding adaptation tempo. The first limitation is in addressing the tempo of temporal distance during model adaption. Most theoretical work \cite{fei2020dynamic,mao2020model,cheung2019learning} focuses on the fixed or full reference length of the past to estimate and adapt the model. \cite{zhao2021adaptivity,zhou2020nonstationary} have addressed the relationship between environment tempo and online optimization by time-varying step size, but these works are limited to the convex optimization or fixed transition probability of online MDP. We demonstrate that the optimal tempo of the temporal distance, denoted as sliding window length, depends on the tempo of the environment, denoted as the total variation budget. 
The second issue is relationship between model update tempo and policy update tempo. Most existing works \cite{chen2022adaptive,huang2021adarl,feng2022factored,zintgraf2019varibad,nagabandi2018deep,hafner2023mastering} that learn the model and optimize the policy have not addressed how accurately fit the model can influence how much policy needs to be updated at current environment. We demonstrate that the tempo of model update, denoted as model accuracy error, influences the tempo of policy optimization, denoted as iteration of policy optimization.
\hyunin{I moved the second issue and third issue that Yuhao mentioned to appendix. I think aligning the existing works' limitations regarding with tempo is important in main paper.}



\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/motivation_2dreacher_2.png}
    \caption{(a) 2D goal reacher in time-varying environment (b) forecasted model-based synthetic trajectories (c) Rewards per episode in 2D goal reacher with four model-free baselines. \texttt{F-MBPO}$^{*}$ is our proposed method (d) the average success rate of Pro-OLS, proactive model-free method, for five different speeds and five different learning rates }
    \label{fig:fig1}
\end{figure}


Our approach to finding a good tempo trade-off between the algorithm and the environment is to introduce our \textbf{ meta-framework}. Our meta framework  modifies the agent's algorithm by \textbf{conditioning} on the forecasted environment tempo and then solely solves the modified algorithm's optimization problem that is \textbf{independent} to any nonstationary environment factors. 

To be specific, let us take a toy example that a robot is given a task to reach inside a gray-shaded target box where its position changes as time goes by (Figure \ref{fig:fig1}-(a)). Figure \ref{fig:fig1}-(d) shows that finding a good learning rate adaptive to the target box speed of the model-free method is difficult and also supports stereotype intuition needs to be modified: faster speed requires small learning rates. This is because some hidden factors exist that were not considered in the trade-off between learning rates and target box speed, such as stocacity of environment, or number of policy iterations, etc. However, after the robot finishes execution at episode 10, if the robot can $observe$ how the box changes during episode 7 to 10, then predicts its position for the next episode, then the robot can obtain good $\pi_{11}$ \textit{in advance} at current episode 10. Namely, the robot's strategy is that 1) creates the future model conditioned on the forecasted box position of next episode, then 2) solves the policy optimization problem in that model, which now does not depends on any non-stationary environment factors from environment. This strategy can be also viewed as rather than directly solving the non-stationary optimization problem at current time, it proactively foresees where the next episode's target box will be located and solves the temporal stationary optimization in that created forecasted environment.

Our idea, utilizing the forecasted environments to generate multiple consistent synthetic samples for policy optimization, can provide robust and better gradient directions of policy than the existing works \cite{chandak2020optimizing,al2017continuous,finn2019online} (figure \ref{fig:fig1}-(b)), which is well supported by simulation results of the 2D goal reacher in Figure \ref{fig:fig1}-(c). In the non-stationary environment, the agent usually obtains a trajectory from the current environment since the environment is constantly changing, which is challenging to optimize the policy using only a single trajectory. To solve this issue, if the agent updates its policy based on historical trajectories in a non-stationary environment, a lag between the environment with which the agent has interacted and the environment in which the agent has to optimized leads to inaccurate estimation of loss function and yields an undesired policy. 
However, if the agent is able to maintain an accurate foresight of the future environment and utilize the forecasted environment to generate the multiple synthetic trajectories, then the foresight of the environment and unlimited number of synthetic trajectories will empower the agent to adapt its policy quickly for every future environment. Namely, a more accurate forecasting the future environment, much lower the model prediction error between forecasted environment and true future environment, then multiple samples from forecasted environment  enables the agent to optimize policy multiple iterations for each certain environment, which reduces the optimallity gap compared with the one-step policy optimization method. Those two in combination can provide a tighter dynamic regret. We elaborate specific details in Appendix \ref{appendix: 2D reacher environment setting}, \ref{appendix : Theoretical_Motivation}. 

As motivated by the previous toy example, we aim to develop a systematic approach to fully leverage the proactive model forecaster and the synthetic samples from the forecasted envirments to obtain the optimal future policy in advance at the current episode.


In this paper, we propose a fast adaptation strategy, \textbf{proactive model-based model-free} meta framework, that can be applied with any classical RL algorithm. The proposed meta framework is characterized by three key features: 1) it is \textit{proactive} in nature as it forecasts the future MDP; 2) it is \textit{model-based} by creating a synthetic future MDP; then 3) it is \textit{model-free} by directly optimizing the policy in the synthetic environment and using it in the subsequent future episode. To deeply understand and characterize our meta framework, we further propose two specific instances of our proposed meta framework : \texttt{FT-MBPO}, a theoretical instance for tabular environments, and \texttt{F-MBPO}, the practical instance for complex environments. 

The contribution of our work is listed below.
\begin{enumerate}
    \item \textbf{Generality : } our meta framework to cope with non-stationary environments that could be equipped with RL algorithms. This is supported by Theorem \ref{thm:2}, Remark \ref{rmk:W-LSE_modelerror}.
    \item \textbf{Theoretical analysis (Section \ref{From_FT-MBPO_to_F-MBPO}): }
    \begin{itemize}
        \item we provide the dynamic regret of \texttt{FT-MBPO} in Theorem \ref{thm:forecasteddynamicregret}.
        \item we show that a good baseline RL algorithm is not enough to obtain sublinear dynamic regret in Proposition \ref{proposition:1} by pointing out that dynamic regret depends on our meta framework in Remark $\ref{remark:1}$.
        \item we show the dynamic regret achieves sublinearity when using the well-known non-stationary estimator in Theorem \ref{thm:2}, and can be more improved by a more general non-stationary estimator that includes a joint-optimization problem in Remark \ref{rmk:W-LSE_modelerror}.
    \end{itemize}
    \item \textbf{Practical implementation (Section \ref{experiments}): }
   
    \begin{itemize}
        \item  we conduct experiments of \texttt{F-MBPO} on three different Mujoco tasks and verify that our meta framework can quickly adapt and outform than the $\{\text{proactive, reactive}\}$-model-free methods proposed to solve the non-stationary MDPs and the typical model-based model-free method proposed to solve the statinoary MDPs.
    \end{itemize}
\end{enumerate}

This paper is organized as follows. Section \ref{problem_statement_and_background} provides the necessary background on non-stationary MDPs. In section \ref{method}, we introduce our main contribution, the meta framework that forecasts future MDPs. In section \ref{From_FT-MBPO_to_F-MBPO}, we then present two specific algorithms, FT-MBPO and F-MBPO, and provide theoretical analysis that leads to practical insights for algorithm design. Finally, we present our experimental results in section \ref{experiments}.


